SimCADO - an instrument data simulator package for MICADO at the E-ELT

MICADO will be the first-light wide-field imager for the European Extremely Large Telescope (E-ELT) and will provide difiraction limited imaging (7mas at 1.2mm) over a ~53 arcsecond field of view. In order to support various consortium activities we have developed a first version of SimCADO: an instrument simulator for MICADO. SimCADO uses the results of the detailed simulation efforts conducted for each of the separate consortium-internal work packages in order to generate a model of the optical path from source to detector readout. SimCADO is thus a tool to provide scientific context to both the science and instrument development teams who are ultimately responsible for the final design and future capabilities of the MICADO instrument. Here we present an overview of the inner workings of SimCADO and outline our plan for its further development.

==> 5_examples.tex <==
\section{Use Case Example and Results} 
\label{sec:results}

Use case examples

\subsection{Stellar population}
* Crowded fields
    * Accurate photometry
\subsection{Galaxy}

